Learning View-Dependent Splatting Kernels

We present a differentiable framework to automatically learn view-dependent 2D kernels in a splatting-based pipeline to improve reconstruction quality and representation efficiency for novel 3D view synthesis. Our volumetric primitive is defined as a bounding ellipsoid and a 3D-kernel latent vector. We first learn a projection network to output a 2D-kernel latent, taking the attributes of the ellipsoid and the 3D-kernel latent as input. Next, the result is sent to a decoder to produce a radially symmetric 2D kernel in terms of Mahalanobis distance, bounded by the projected ellipsoid. The neural networks along with per-primitive attributes are jointly optimized. The effectiveness of our approach is demonstrated on standard benchmarks, comparing favorably against state-of-the-art techniques on both analytical and learned kernels. Finally, we extend the idea to learn general 2D kernels for 2D splatting as well as image representation.

==> fig/abl_table_K.tex <==
% \begin{table}[h]
% \centering
% \resizebox{\columnwidth}{!}{% 
% \begin{tabular}{c|cc|cc|cc}
% \toprule
% \multirow{2}{*}{Prim. Count} & \multicolumn{2}{c|}{$K=2$} & \multicolumn{2}{c|}{$K=4$} & \multicolumn{2}{c}{$K=8$} \\
%  & PSNR$\uparrow$ & FPS$\uparrow$ & PSNR$\uparrow$ & FPS$\uparrow$ & PSNR$\uparrow$ & FPS$\uparrow$ \\
% \midrule
% % Sparse Regime: K=8 收益巨大，FPS 只有轻微损耗
% 0.1 M & 26.15 & 210 & 27.80 & 198 & 28.12 & 185 \\ 
% % Medium Regime: 过渡带
% 0.5 M & 29.50 & 145 & 29.95 & 138 & 30.08 & 128 \\ 
% % Dense Regime: K=2 足够，FPS 随 K 增加而下降
% 1.5 M & 31.20 & 62 & 31.24 & 58 & 31.25 & 53 \\ 
% \bottomrule
% \end{tabular}
% }
% \vspace{3pt}
% \caption{Ablation study on the Anchor Points Distilling Strategy using Mip-NeRF 360 Indoor scenes. We evaluate PSNR and Rendering Speed (FPS) across different primitive counts (Regimes) and anchor point quantities ($k$).}
% \label{tab:ablation_K}

% \end{table}

==> fig/density_visualization.tex <==
% \begin{figure*}[htbp]
%     \centering
%     \captionsetup[subfigure]{justification=centering}

%     % ==================================================
%     % 定义列宽
%     % GT (3:2): 0.32
%     % Ours (1:1 + small): 0.16
%     % Merged (Big Image): 0.49 (约等于3个Ours宽)
%     % ==================================================
%     \newcommand{\colGT}{0.32\linewidth}
%     \newcommand{\colOurs}{0.16\linewidth}
%     \newcommand{\colMerge}{0.49\linewidth}

%     % ==========================
%     % 1. 标题行 (Header Row)
%     % ==========================
%     \begin{minipage}{\textwidth}
%         \begin{minipage}{0.10in}
%             \hspace{0.03in} 
%         \end{minipage}  
%         \begin{minipage}{\dimexpr\textwidth-0.03in-1em\relax}
%             \centering
%             % 1. GT
%             \begin{minipage}{\colGT} \centering \subcaption*{\small scene} \end{minipage}%
%             \hfill
%             % 2. Ours
%             \begin{minipage}{\colOurs} \centering \subcaption*{\small Ours} \end{minipage}%
%             \hfill
%             % 3. Merged (统称为 Baselines)
%             \begin{minipage}{\colMerge} \centering \subcaption*{\small multiview statistic} \end{minipage}
%         \end{minipage}       
%     \end{minipage}
    
%     \vspace{2pt} 

%     % ==========================
%     % 2. 第一行数据 (Room)
%     % ==========================
%     \begin{minipage}{\textwidth}
%         % --- 左侧竖排标签 ---
%         \begin{minipage}[t]{0.10in}    
%             \vspace{0.6in} % 这个值可能需要根据实际图片高度微调以垂直居中
%             \centering
%             \rotatebox{90}{\small \textsc{Room}}
%         \end{minipage}
%         % --- 右侧图片内容 ---
%         \begin{minipage}[t]{\dimexpr\textwidth-0.03in-1em\relax}
%             \vspace{0pt}
%             \centering
            
%             % [第1列 GT]
%             % 3:2 比例 -> 高度约为 0.66 * 0.32 = 0.21，与 Ours高度基本一致
%             \begin{minipage}[t]{\colGT}
%                 \vspace{0pt}
%                 \centering
%                 \includegraphics[width=\linewidth, height=0.66\linewidth]{imgs/comparison/room/room_our_13.png}
%             \end{minipage}%
%             \hfill
%             % [第2列 Ours] (复合结构：上大下小)
%             \begin{minipage}[t]{\colOurs}
%                 \vspace{0pt}
%                 \centering
%                 % 主图 (方形)
%                 \includegraphics[width=\linewidth, height=\linewidth]{imgs/stats/room/trend_view0.pdf}
%                 \put(-13,3){\scalebox{.6}{\color{black} 0.9}}
%                 \vspace{1.5pt} 
%                 % 底部三张小曲线图
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{imgs/stats/room/bell_curve_orbit_cam_0_2732.pdf}\hfill
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{imgs/stats/room/bell_curve_orbit_cam_1_9845.pdf}\hfill
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{imgs/stats/room/bell_curve_orbit_cam_2_3264.pdf}
%             \end{minipage}%
%             \hfill
%             % [第3列 Merged Baselines] (单张大图)
%             % 这里的图片包含了 MCMC/DBS/SSS 的所有内容
%             \begin{minipage}[t]{\colMerge}
%                 \vspace{0pt}
%                 \centering
%                 % 关键参数：height=0.44\linewidth
%                 % 这个高度系数确保了这张长图的高度 = 左侧 Ours 列的总高度 (大图+间隙+小图)
%                 \includegraphics[width=\linewidth, height=0.44\linewidth]{imgs/stats/room/violin_8view.pdf}
%             \end{minipage}
%         \end{minipage}
%     \end{minipage}

%     \vspace{4pt} % 行间距

%     % ==========================
%     % 3. 第二行数据 (Bonsai)
%     % ==========================
%     \begin{minipage}{\textwidth}
%         % --- 左侧竖排标签 ---
%         \begin{minipage}[t]{0.10in}    
%             \vspace{0.6in} % 这个值可能需要根据实际图片高度微调以垂直居中
%             \centering
%             \rotatebox{90}{\small \textsc{bonsai}}
%         \end{minipage}
%         % --- 右侧图片内容 ---
%         \begin{minipage}[t]{\dimexpr\textwidth-0.03in-1em\relax}
%             \vspace{0pt}
%             \centering
            
%             % [第1列 GT]
%             % 3:2 比例 -> 高度约为 0.66 * 0.32 = 0.21，与 Ours高度基本一致
%             \begin{minipage}[t]{\colGT}
%                 \vspace{0pt}
%                 \centering
%                 \includegraphics[width=\linewidth, height=0.66\linewidth]{imgs/comparison/bonsai/bonsai_our_08.png}
%             \end{minipage}%
%             \hfill
%             % [第2列 Ours] (复合结构：上大下小)
%             \begin{minipage}[t]{\colOurs}
%                 \vspace{0pt}
%                 \centering
%                 % 主图 (方形)
%                 \includegraphics[width=\linewidth, height=\linewidth]{imgs/stats/bonsai/trend_view0.pdf}
%                 \put(-13,3){\scalebox{.6}{\color{black} 0.9}}
%                 \vspace{1.5pt} 
%                 % 底部三张小曲线图
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{imgs/stats/bonsai/bell_curve_orbit_cam_0_2732.pdf}\hfill
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{imgs/stats/bonsai/bell_curve_orbit_cam_1_9845.pdf}\hfill
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{imgs/stats/bonsai/bell_curve_orbit_cam_2_3264.pdf}
%             \end{minipage}%
%             \hfill
%             % [第3列 Merged Baselines] (单张大图)
%             % 这里的图片包含了 MCMC/DBS/SSS 的所有内容
%             \begin{minipage}[t]{\colMerge}
%                 \vspace{0pt}
%                 \centering
%                 % 关键参数：height=0.44\linewidth
%                 % 这个高度系数确保了这张长图的高度 = 左侧 Ours 列的总高度 (大图+间隙+小图)
%                 \includegraphics[width=\linewidth, height=0.44\linewidth]{imgs/stats/bonsai/violin_8view.pdf}
%             \end{minipage}
%         \end{minipage}
%     \end{minipage}

%     \vspace{4pt} 

%     % ==========================
%     % 4. 第三行数据 (Train)
%     % ==========================
%     \begin{minipage}{\textwidth}
%         % --- 左侧竖排标签 ---
%         \begin{minipage}[t]{0.10in}    
%             \vspace{0.6in} % 这个值可能需要根据实际图片高度微调以垂直居中
%             \centering
%             \rotatebox{90}{\small \textsc{train}}
%         \end{minipage}
%         % --- 右侧图片内容 ---
%         \begin{minipage}[t]{\dimexpr\textwidth-0.03in-1em\relax}
%             \vspace{0pt}
%             \centering
            
%             % [第1列 GT]
%             % 3:2 比例 -> 高度约为 0.66 * 0.32 = 0.21，与 Ours高度基本一致
%             \begin{minipage}[t]{\colGT}
%                 \vspace{0pt}
%                 \centering
%                 \includegraphics[width=\linewidth, height=0.66\linewidth]{imgs/comparison/train/train_our_06.png}
%             \end{minipage}%
%             \hfill
%             % [第2列 Ours] (复合结构：上大下小)
%             \begin{minipage}[t]{\colOurs}
%                 \vspace{0pt}
%                 \centering
%                 % 主图 (方形)
%                 \includegraphics[width=\linewidth, height=\linewidth]{imgs/stats/train/trend_view0.pdf}
%                 \put(-13,3){\scalebox{.6}{\color{black} 0.9}}
%                 \vspace{1.5pt} 
%                 % 底部三张小曲线图
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{imgs/stats/train/bell_curve_orbit_cam_0_2732.pdf}\hfill
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{imgs/stats/train/bell_curve_orbit_cam_1_9845.pdf}\hfill
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{imgs/stats/train/bell_curve_orbit_cam_2_3264.pdf}
%             \end{minipage}%
%             \hfill
%             % [第3列 Merged Baselines] (单张大图)
%             % 这里的图片包含了 MCMC/DBS/SSS 的所有内容
%             \begin{minipage}[t]{\colMerge}
%                 \vspace{0pt}
%                 \centering
%                 % 关键参数：height=0.44\linewidth
%                 % 这个高度系数确保了这张长图的高度 = 左侧 Ours 列的总高度 (大图+间隙+小图)
%                 \includegraphics[width=\linewidth, height=0.44\linewidth]{imgs/stats/train/violin_8view.pdf}
%             \end{minipage}
%         \end{minipage}
%     \end{minipage}

%     % ==========================
%     % 4. 第三行数据 (Playroom)
%     % ==========================
%     \begin{minipage}{\textwidth}
%         % --- 左侧竖排标签 ---
%         \begin{minipage}[t]{0.10in}    
%             \vspace{0.6in} % 这个值可能需要根据实际图片高度微调以垂直居中
%             \centering
%             \rotatebox{90}{\small \textsc{playroom}}
%         \end{minipage}
%         % --- 右侧图片内容 ---
%         \begin{minipage}[t]{\dimexpr\textwidth-0.03in-1em\relax}
%             \vspace{0pt}
%             \centering
            
%             % [第1列 GT]
%             % 3:2 比例 -> 高度约为 0.66 * 0.32 = 0.21，与 Ours高度基本一致
%             \begin{minipage}[t]{\colGT}
%                 \vspace{0pt}
%                 \centering
%                 \includegraphics[width=\linewidth, height=0.66\linewidth]{imgs/comparison/playroom/playroom_our_02.png}
%             \end{minipage}%
%             \hfill
%             % [第2列 Ours] (复合结构：上大下小)
%             \begin{minipage}[t]{\colOurs}
%                 \vspace{0pt}
%                 \centering
%                 % 主图 (方形)
%                 \includegraphics[width=\linewidth, height=\linewidth]{imgs/stats/playroom/trend_view0.pdf}
%                 \put(-13,3){\scalebox{.6}{\color{black} 0.9}}
%                 \vspace{1.5pt} 
%                 % 底部三张小曲线图
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{imgs/stats/playroom/bell_curve_orbit_cam_0_2732.pdf}\hfill
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{imgs/stats/playroom/bell_curve_orbit_cam_1_9845.pdf}\hfill
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{imgs/stats/playroom/bell_curve_orbit_cam_2_3264.pdf}
%             \end{minipage}%
%             \hfill
%             % [第3列 Merged Baselines] (单张大图)
%             % 这里的图片包含了 MCMC/DBS/SSS 的所有内容
%             \begin{minipage}[t]{\colMerge}
%                 \vspace{0pt}
%                 \centering
%                 % 关键参数：height=0.44\linewidth
%                 % 这个高度系数确保了这张长图的高度 = 左侧 Ours 列的总高度 (大图+间隙+小图)
%                 \includegraphics[width=\linewidth, height=0.44\linewidth]{imgs/stats/playroom/violin_8view.pdf}
%             \end{minipage}
%         \end{minipage}
%     \end{minipage}
    
%     \caption{Visual comparisons. The last column is a single image summarizing the baseline methods.}
%     \label{fig:fully_merged}
% \end{figure*}

==> fig/density_visualization_2.tex <==
% \begin{figure*}[htbp]
%     \centering
%     \captionsetup[subfigure]{justification=centering}
%     \setlength{\tabcolsep}{0pt} % 清除额外间距，完全由我们控制

%     % ==================================================
%     % 核心宽度定义 (基于高度对齐计算)
%     % 设基础正方形边长(高度)为 H
%     % Col 3-5 (1:1): 宽度 = H  -> 设为 0.20
%     % Col 1   (3:2): 宽度 = 1.5H -> 设为 0.30
%     % Col 2   (4张竖排): 宽度 = 0.25H -> 设为 0.05
%     % 总和: 0.30 + 0.05 + 3*0.20 = 0.95 (剩余 5% 用于间隙)
%     % ==================================================
%     \newcommand{\colScene}{0.30\linewidth}
%     \newcommand{\colVert}{0.05\linewidth} % 关键：这一列必须非常窄，叠起来才不会太高
%     \newcommand{\colStat}{0.20\linewidth}

%     % ==========================
%     % 1. 标题行 (Header)
%     % ==========================
%     \begin{minipage}{\textwidth}
%         \begin{minipage}{0.02\textwidth} \hspace{0pt} \end{minipage}  
%         \begin{minipage}{0.975\textwidth}
%             \centering
%             \begin{minipage}{\colScene} \centering \subcaption*{\small Scene} \end{minipage}\hfill
%             \begin{minipage}{\colVert} \centering \subcaption*{\tiny Trend} \end{minipage}\hfill
%             \begin{minipage}{\colStat} \centering \subcaption*{\small View0} \end{minipage}\hfill
%             \begin{minipage}{\colStat} \centering \subcaption*{\small View1} \end{minipage}\hfill
%             \begin{minipage}{\colStat} \centering \subcaption*{\small View2} \end{minipage}
%         \end{minipage}       
%     \end{minipage}
    
%     \vspace{2pt} 

%     % ==========================
%     % 2. 第一行数据 (Room)
%     % ==========================
%     \begin{minipage}{\textwidth}
%         % 左侧标签
%         \begin{minipage}[c]{0.02\textwidth}    
%             \centering
%             \rotatebox{90}{\small \textsc{Room}}
%         \end{minipage}
%         % 右侧内容 (使用 [c] 垂直居中对齐)
%         \begin{minipage}[c]{0.975\textwidth}
%             \centering
            
%             % [Col 1] 3:2 大图
%             % height 设为 0.666 宽度，确保比例正确
%             \begin{minipage}[c]{\colScene}
%                 \centering
%                 \includegraphics[width=\linewidth, height=0.666\linewidth]{imgs/comparison/room/room_gt.png}
%             \end{minipage}\hfill
%             % [Col 2] 竖排 4 张小图
%             % 这一列宽度设为 0.05 后，4张图叠起来的高度约为 0.05*4 = 0.20，与右边对齐
%             \begin{minipage}[c]{\colVert}
%                 \centering
%                 \setlength{\lineskip}{1pt} % 图片垂直间距
%                 \includegraphics[width=\linewidth, height=\linewidth]{imgs/stats/room/bell_curve_orbit_cam_0_2732.pdf}
%                 \includegraphics[width=\linewidth, height=\linewidth]{imgs/stats/room/bell_curve_orbit_cam_1_9845.pdf}
%                 \includegraphics[width=\linewidth, height=\linewidth]{imgs/stats/room/bell_curve_orbit_cam_2_3264.pdf}
%                 \includegraphics[width=\linewidth, height=\linewidth]{imgs/stats/room/bell_curve_orbit_cam_3_4859.pdf}
%             \end{minipage}\hfill
%             % [Col 3] 正方形
%             \begin{minipage}[c]{\colStat}
%                 \centering
%                 \includegraphics[width=\linewidth, height=\linewidth]{imgs/stats/room/heatmap_view0.pdf}
%             \end{minipage}\hfill
%             % [Col 4] 正方形
%             \begin{minipage}[c]{\colStat}
%                 \centering
%                 \includegraphics[width=\linewidth, height=\linewidth]{imgs/stats/room/heatmap_view2.pdf}
%             \end{minipage}\hfill
%             % [Col 5] 正方形
%             \begin{minipage}[c]{\colStat}
%                 \centering
%                 \includegraphics[width=\linewidth, height=\linewidth]{imgs/stats/room/heatmap_view3.pdf}
%             \end{minipage}
%         \end{minipage}
%     \end{minipage}

%     \vspace{4pt}

%     % ==========================
%     % 3. 第二行数据 (Bonsai)
%     % ==========================
%     \begin{minipage}{\textwidth}
%         % 左侧标签
%         \begin{minipage}[c]{0.02\textwidth}    
%             \centering
%             \rotatebox{90}{\small \textsc{bonsai}}
%         \end{minipage}
%         % 右侧内容 (使用 [c] 垂直居中对齐)
%         \begin{minipage}[c]{0.975\textwidth}
%             \centering
            
%             % [Col 1] 3:2 大图
%             % height 设为 0.666 宽度，确保比例正确
%             \begin{minipage}[c]{\colScene}
%                 \centering
%                 \includegraphics[width=\linewidth, height=0.666\linewidth]{imgs/comparison/bonsai/bonsai_gt_26.png}
%             \end{minipage}\hfill
%             % [Col 2] 竖排 4 张小图
%             % 这一列宽度设为 0.05 后，4张图叠起来的高度约为 0.05*4 = 0.20，与右边对齐
%             \begin{minipage}[c]{\colVert}
%                 \centering
%                 \setlength{\lineskip}{1pt} % 图片垂直间距
%                 \includegraphics[width=\linewidth, height=\linewidth]{imgs/stats/bonsai/bell_curve_orbit_cam_0_2732.pdf}
%                 \includegraphics[width=\linewidth, height=\linewidth]{imgs/stats/bonsai/bell_curve_orbit_cam_1_9845.pdf}
%                 \includegraphics[width=\linewidth, height=\linewidth]{imgs/stats/bonsai/bell_curve_orbit_cam_2_3264.pdf}
%                 \includegraphics[width=\linewidth, height=\linewidth]{imgs/stats/bonsai/bell_curve_orbit_cam_3_4859.pdf}
%             \end{minipage}\hfill
%             % [Col 3] 正方形
%             \begin{minipage}[c]{\colStat}
%                 \centering
%                 \includegraphics[width=\linewidth, height=\linewidth]{imgs/stats/bonsai/heatmap_view0.pdf}
%             \end{minipage}\hfill
%             % [Col 4] 正方形
%             \begin{minipage}[c]{\colStat}
%                 \centering
%                 \includegraphics[width=\linewidth, height=\linewidth]{imgs/stats/bonsai/heatmap_view2.pdf}
%             \end{minipage}\hfill
%             % [Col 5] 正方形
%             \begin{minipage}[c]{\colStat}
%                 \centering
%                 \includegraphics[width=\linewidth, height=\linewidth]{imgs/stats/bonsai/heatmap_view3.pdf}
%             \end{minipage}
%         \end{minipage}
%     \end{minipage}
    
%     % ==========================
%     % 3. 第二行数据 (Bonsai)
%     % ==========================

%     \begin{minipage}{\textwidth}
%         % 左侧标签
%         \begin{minipage}[c]{0.02\textwidth}    
%             \centering
%             \rotatebox{90}{\small \textsc{playroom}}
%         \end{minipage}
%         % 右侧内容 (使用 [c] 垂直居中对齐)
%         \begin{minipage}[c]{0.975\textwidth}
%             \centering
            
%             % [Col 1] 3:2 大图
%             % height 设为 0.666 宽度，确保比例正确
%             \begin{minipage}[c]{\colScene}
%                 \centering
%                 \includegraphics[width=\linewidth, height=0.666\linewidth]{imgs/comparison/playroom/playroom_gt_06.png}
%             \end{minipage}\hfill
%             % [Col 2] 竖排 4 张小图
%             % 这一列宽度设为 0.05 后，4张图叠起来的高度约为 0.05*4 = 0.20，与右边对齐
%             \begin{minipage}[c]{\colVert}
%                 \centering
%                 \setlength{\lineskip}{1pt} % 图片垂直间距
%                 \includegraphics[width=\linewidth, height=\linewidth]{imgs/stats/playroom/bell_curve_orbit_cam_0_2732.pdf}
%                 \includegraphics[width=\linewidth, height=\linewidth]{imgs/stats/playroom/bell_curve_orbit_cam_1_9845.pdf}
%                 \includegraphics[width=\linewidth, height=\linewidth]{imgs/stats/playroom/bell_curve_orbit_cam_2_3264.pdf}
%                 \includegraphics[width=\linewidth, height=\linewidth]{imgs/stats/playroom/bell_curve_orbit_cam_3_4859.pdf}
%             \end{minipage}\hfill
%             % [Col 3] 正方形
%             \begin{minipage}[c]{\colStat}
%                 \centering
%                 \includegraphics[width=\linewidth, height=\linewidth]{imgs/stats/playroom/histogram_view0.pdf}
%             \end{minipage}\hfill
%             % [Col 4] 正方形
%             \begin{minipage}[c]{\colStat}
%                 \centering
%                 \includegraphics[width=\linewidth, height=\linewidth]{imgs/stats/playroom/histogram_view2.pdf}
%             \end{minipage}\hfill
%             % [Col 5] 正方形
%             \begin{minipage}[c]{\colStat}
%                 \centering
%                 \includegraphics[width=\linewidth, height=\linewidth]{imgs/stats/playroom/histogram_view4.pdf}
%             \end{minipage}
%         \end{minipage}
%     \end{minipage}

%     % ==========================
%     % 3. 第二行数据 (Bonsai)
%     % ==========================

%     \begin{minipage}{\textwidth}
%         % 左侧标签
%         \begin{minipage}[c]{0.02\textwidth}    
%             \centering
%             \rotatebox{90}{\small \textsc{train}}
%         \end{minipage}
%         % 右侧内容 (使用 [c] 垂直居中对齐)
%         \begin{minipage}[c]{0.975\textwidth}
%             \centering
            
%             % [Col 1] 3:2 大图
%             % height 设为 0.666 宽度，确保比例正确
%             \begin{minipage}[c]{\colScene}
%                 \centering
%                 \includegraphics[width=\linewidth, height=0.666\linewidth]{imgs/comparison/train/box_train_gt_08.png}
%             \end{minipage}\hfill
%             % [Col 2] 竖排 4 张小图
%             % 这一列宽度设为 0.05 后，4张图叠起来的高度约为 0.05*4 = 0.20，与右边对齐
%             \begin{minipage}[c]{\colVert}
%                 \centering
%                 \setlength{\lineskip}{1pt} % 图片垂直间距
%                 \includegraphics[width=\linewidth, height=\linewidth]{imgs/stats/train/bell_curve_orbit_cam_0_2732.pdf}
%                 \includegraphics[width=\linewidth, height=\linewidth]{imgs/stats/train/bell_curve_orbit_cam_1_9845.pdf}
%                 \includegraphics[width=\linewidth, height=\linewidth]{imgs/stats/train/bell_curve_orbit_cam_2_3264.pdf}
%                 \includegraphics[width=\linewidth, height=\linewidth]{imgs/stats/train/bell_curve_orbit_cam_3_4859.pdf}
%             \end{minipage}\hfill
%             % [Col 3] 正方形
%             \begin{minipage}[c]{\colStat}
%                 \centering
%                 \includegraphics[width=\linewidth, height=\linewidth]{imgs/stats/train/histogram_view0.pdf}
%             \end{minipage}\hfill
%             % [Col 4] 正方形
%             \begin{minipage}[c]{\colStat}
%                 \centering
%                 \includegraphics[width=\linewidth, height=\linewidth]{imgs/stats/train/histogram_view2.pdf}
%             \end{minipage}\hfill
%             % [Col 5] 正方形
%             \begin{minipage}[c]{\colStat}
%                 \centering
%                 \includegraphics[width=\linewidth, height=\linewidth]{imgs/stats/train/histogram_view4.pdf}
%             \end{minipage}
%         \end{minipage}
%     \end{minipage}
    
%     \caption{Visual comparisons. Note that the narrow second column aligns in height with the surrounding columns due to stacking 4 images.}
%     \label{fig:aligned_rows}
% \end{figure*}

==> fig/detail_quantitive.tex <==
\begin{minipage}{\textwidth}
\centering
\captionsetup{type=table}
\captionof{table}{Per-scene reconstruction quality of our approach and state-of-the-art techniques~(3DGS-MCMC~\cite{kheradmand20243dgsmcmc}, SSS~\cite{zhu2025sss} and DBS~\cite{liu2025deformablebetasplatting}) on 4 standard datasets: Mip-NeRF360~\cite{barron2022mipnerf360}, Tanks~\&~Temples~\cite{Tank&Temple}, Deep Blending~\cite{DeepBlending2018} and NeRF Synthetic~\cite{mildenhall2020nerf}. Baseline results are obtained from the original papers whenever available; otherwise, we run the official implementation and list the results in \textit{italics}. SH = spherical harmonics, SB = spherical Beta, T~\&~T = Tanks~\&~Temples, DB = Deep Blending.
% In both 3D/2D splatting, our approach is the \emph{best or second-best} in all quality metrics across all benchmarks. Please also see the supplemental material for a . For qualitative comparisons between some top performing approaches, please refer to~\cref{fig:main_compact} as well as the accompanying video
}
\label{tab:per_scene_eval_5methods}
\vspace{0.5em}
\resizebox{\textwidth}{!}{%
\setlength{\tabcolsep}{4pt}
\renewcommand{\arraystretch}{1.2}
\begin{tabular}{cl|c|c|c|c|c}
\toprule
\multicolumn{2}{c|}{Scenes} & 3DGS-MCMC & SSS & DBS & Ours~(3D+SH) & Ours~(3D+SB) \\
\midrule
\multirow{10}{*}{\rotatebox{90}{Mip-NeRF 360}} 
& bicycle & 26.15 / 0.81 / 0.18 & 25.68 / 0.798 / 0.173 & 26.04 / 0.804 / 0.169 & 26.00 / 0.797 / 0.187 & 25.95 / 0.795 / 0.200 \\
& flowers & 22.12 / 0.642 / 0.31 & \textit{21.77 / 0.629 / 0.302} & 22.44 / 0.650 / 0.308 & 22.47 / 0.644 / 0.299 & 22.34 / 0.641 / 0.307 \\
& garden  & 28.16 / 0.89 / 0.10 & 28.09 / 0.882 / 0.009 & 28.15 / 0.882 / 0.096 & 28.07 / 0.878 / 0.096 & 28.09 / 0.877 / 0.100 \\
& stump   & 27.80 / 0.82 / 0.19 & 27.17 / 0.813 / 0.174 & 27.56 / 0.815 / 0.184 & 27.80 / 0.813 / 0.186 & 27.62 / 0.807 / 0.193 \\
& treehill& 23.31 / 0.66 / 0.29 & \textit{23.19 / 0.661 / 0.300} & 23.49 / 0.676 / 0.293 & 23.54 / 0.674 / 0.317 & 23.60 / 0.671 / 0.326 \\
& room    & 32.48 / 0.94 / 0.25 & 32.57 / 0.938 / 0.167 & 32.83 / 0.941 / 0.168 & 33.58 / 0.943 / 0.165 & 33.59 / 0.943 / 0.167 \\
& counter & 29.51 / 0.92 / 0.22 & 29.87 / 0.926 / 0.156 & 30.36 / 0.930 / 0.154 & 30.51 / 0.931 / 0.154 & 30.74 / 0.931 / 0.152 \\
& kitchen & 32.27 / 0.94 / 0.14 & 32.43 / 0.939 / 0.104 & 32.61 / 0.939 / 0.110 & 32.61 / 0.939 / 0.108 & 32.79 / 0.939 / 0.108 \\
& bonsai  & 32.88 / 0.95 / 0.22 & 33.50 / 0.956 / 0.151 & 33.90 / 0.957 / 0.156 & 34.05 / 0.959 / 0.153 & 34.69 / 0.959 / 0.152 \\
& average & 28.29 / 0.84 / 0.21 & \textit{28.25 / 0.838 / 0.171} & 28.60 / 0.844 / 0.182 & 28.73 / 0.842 / 0.185 & 28.82 / 0.840 / 0.189 \\
\midrule
\multirow{9}{*}{\rotatebox{90}{NeRF Synthetic}} 
& chair    & 36.51 / 0.99 / 0.02 & \textit{36.64 / 0.990 / 0.010} & 36.74 / 0.990 / 0.010 & 36.88 / 0.990 / 0.009 & 36.62 / 0.990 / 0.009 \\
& drums    & 26.29 / 0.95 / 0.04 & \textit{26.29 / 0.955 / 0.037} & 26.78 / 0.958 / 0.033 & 26.68 / 0.957 / 0.033 & 26.85 / 0.958 / 0.032 \\
& ficus    & 35.07 / 0.99 / 0.01 & \textit{36.60 / 0.989 / 0.011} & 36.75 / 0.990 / 0.010 & 37.05 / 0.990 / 0.009 & 37.00 / 0.990 / 0.009 \\
& hotdog   & 37.82 / 0.99 / 0.02 & \textit{38.55 / 0.987 / 0.018} & 38.85 / 0.988 / 0.015 & 38.77 / 0.988 / 0.015 & 38.45 / 0.987 / 0.015 \\
& lego     & 36.01 / 0.98 / 0.02 & \textit{36.74 / 0.985 / 0.015} & 37.12 / 0.985 / 0.014 & 36.99 / 0.985 / 0.014 & 37.10 / 0.985 / 0.014 \\
& materials& 30.59 / 0.96 / 0.04 & \textit{30.78 / 0.964 / 0.034} & 31.12 / 0.966 / 0.032 & 31.33 / 0.968 / 0.030 & 31.25 / 0.967 / 0.028 \\
& mic      & 37.29 / 0.99 / 0.01 & \textit{37.02 / 0.993 / 0.006} & 37.66 / 0.994 / 0.005 & 37.76 / 0.994 / 0.005 & 37.26 / 0.994 / 0.005 \\
& ship     & 30.82 / 0.91 / 0.12 & \textit{31.71 / 0.905 / 0.101} & 32.13 / 0.910 / 0.103 & 32.32 / 0.913 / 0.098 & 32.10 / 0.912 / 0.101 \\
& average & 33.80 / 0.97 / 0.04 & \textit{34.29 / 0.971 / 0.029} & 34.64 / 0.973 / 0.028 & 34.72 / 0.973 / 0.027 & 34.58 / 0.973 / 0.027 \\
\midrule
\multirow{3}{*}{\rotatebox{90}{T~\&~T}} 
& truck & 26.11 / 0.89 / 0.14 & 26.41 / 0.897 / 0.109 & 26.44 / 0.897 / 0.110 & 26.94 / 0.902 / 0.105 & 26.97 / 0.902 / 0.107 \\
& train & 22.47 / 0.83 / 0.24 & 23.32 / 0.850 / 0.166 & 23.13 / 0.839 / 0.185 & 23.89 / 0.851 / 0.178 & 23.73 / 0.847 / 0.183 \\
& average  & 24.29 / 0.86 / 0.19 & 24.87 / 0.873 / 0.138 & 24.79 / 0.868 / 0.147 & 25.42 / 0.877 / 0.141 & 25.35 / 0.874 / 0.145 \\
\midrule
\multirow{3}{*}{\rotatebox{90}{DB}} 
& drjohnson & 29.00 / 0.89 / 0.33 & 29.66 / 0.905 / 0.249 & 29.39 / 0.908 / 0.240 & 29.85 / 0.911 / 0.234 & 30.00 / 0.910 / 0.235 \\
& playroom  & 30.33 / 0.90 / 0.31 & 30.47 / 0.909 / 0.245 & 30.82 / 0.912 / 0.240 & 31.20 / 0.915 / 0.231 & 31.08 / 0.915 / 0.240 \\
& average & 29.67 / 0.90 / 0.32 & 30.07 / 0.907 / 0.247 & 30.10 / 0.910 / 0.240 & 30.52 / 0.913 / 0.233 & 30.54 / 0.913 / 0.237 \\
\bottomrule
\end{tabular}
}
\par
\end{minipage}

==> fig/diff_spec.tex <==
% \begin{figure*}[htbp]
%     \centering
%     \begin{minipage}{0.03in}
%         \hspace{0.03in}
%     \end{minipage}	
%     \captionsetup[subfigure]{justification=centering}
%     \begin{minipage}{\linewidth}
%         \centering
%         \begin{minipage}{\textwidth}
%             \centering
%             \begin{minipage}{.24\textwidth}
%                 \centering 
%                 \subcaption*{\small GT}
%             \end{minipage}
%             \begin{minipage}{.24\textwidth}
%                 \centering
%                 \subcaption*{\small RGB}
%             \end{minipage}
%             \begin{minipage}{.24\textwidth}
%                 \centering
%                 \subcaption*{\small Diffuse}
%             \end{minipage}
%             \begin{minipage}{.24\textwidth}
%                 \centering
%                 \subcaption*{\small Specular}
%             \end{minipage}
%             % \begin{minipage}{.245\textwidth}
%             %     \centering
%             %     \subcaption*{\small Per-pixel Loss}
%             % \end{minipage}
%         \end{minipage}
%     \end{minipage}  
%     % \begin{minipage}{\linewidth}
%     %     \centering
%     %     \begin{minipage}{.19\linewidth}
%     %         \centering
%     %         \subcaption*{\small LightPattern}
%     %     \end{minipage}
%     %     \begin{minipage}{.19\linewidth}
%     %         \centering
%     %         \subcaption*{\small MaskPattern}
%     %     \end{minipage}
%     %     \begin{minipage}{.19\linewidth}
%     %         \centering
%     %         \subcaption*{\small Photograph}
%     %     \end{minipage}
%     %     \begin{minipage}{.19\linewidth}
%     %         \centering
%     %         \subcaption*{\small DepthUncertainty}
%     %     \end{minipage}
%     % \end{minipage}
%     \begin{minipage}{\textwidth}
%         \begin{minipage}{0.03in}	
%             \centering
%             \rotatebox{90}{\small \textsc{scene1}}
%         \end{minipage}
%         \begin{minipage}{\linewidth}
%             \centering
%             \begin{minipage}{.24\linewidth}
%                 \centering
%                 \includegraphics[width=\linewidth]{imgs/deposition/gt0.png}
%             \end{minipage}
%             \begin{minipage}{.24\linewidth}
%                 \centering
%                 \includegraphics[width=\linewidth]{example-image-duck}
%             \end{minipage}
%             \begin{minipage}{.24\linewidth}
%                 \centering
%                 \includegraphics[width=\linewidth]{imgs/deposition/diffuse0.png}
%             \end{minipage}
%              \begin{minipage}{.24\linewidth}
%                 \centering
%                 \includegraphics[width=\linewidth]{imgs/deposition/specular0.png}
%             \end{minipage}
%         \end{minipage}
%     \end{minipage}

%     \begin{minipage}{\textwidth}
%         \begin{minipage}{0.03in}	
%             \centering
%             \rotatebox{90}{\small \textsc{scene2}}
%         \end{minipage}
%         \begin{minipage}{\linewidth}
%             \centering
%             \begin{minipage}{.24\linewidth}
%                 \centering
%                 \includegraphics[width=\linewidth]{imgs/deposition/gt1.png}
%             \end{minipage}
%             \begin{minipage}{.24\linewidth}
%                 \centering
%                 \includegraphics[width=\linewidth]{example-image-duck}
%             \end{minipage}
%             \begin{minipage}{.24\linewidth}
%                 \centering
%                 \includegraphics[width=\linewidth]{imgs/deposition/diffuse1.png}
%             \end{minipage}
%              \begin{minipage}{.24\linewidth}
%                 \centering
%                 \includegraphics[width=\linewidth]{imgs/deposition/specular1.png}
%             \end{minipage}
%         \end{minipage}
%     \end{minipage}

%         \begin{minipage}{\textwidth}
%         \begin{minipage}{0.03in}	
%             \centering
%             \rotatebox{90}{\small \textsc{scene3}}
%         \end{minipage}
%         \begin{minipage}{\linewidth}
%             \centering
%             \begin{minipage}{.24\linewidth}
%                 \centering
%                 \includegraphics[width=\linewidth]{example-image-duck}
%             \end{minipage}
%             \begin{minipage}{.24\linewidth}
%                 \centering
%                 \includegraphics[width=\linewidth]{example-image-duck}
%             \end{minipage}
%             \begin{minipage}{.24\linewidth}
%                 \centering
%                 \includegraphics[width=\linewidth]{example-image-duck}
%             \end{minipage}
%              \begin{minipage}{.24\linewidth}
%                 \centering
%                 \includegraphics[width=\linewidth]{example-image-duck}
%             \end{minipage}
%         \end{minipage}
%     \end{minipage}
%     \caption{Light decomposition with neural network.}   
%     \label{fig:LightDecomposition}
% \end{figure*}



==> fig/main_comparison.tex <==
% \begin{figure*}
%     \begin{minipage}{\textwidth}
%         \begin{minipage}{0.03in}
%             \hspace{0.03in}
%         \end{minipage}	
%         \captionsetup[subfigure]{justification=centering}
%         \begin{minipage}{\textwidth}
%             \centering
%             \begin{minipage}{\textwidth}
%                 \centering
%                 \begin{minipage}{.19\textwidth}
%                     \centering
%                     \subcaption*{\small GT}
%                 \end{minipage}
%                 \begin{minipage}{.19\textwidth}
%                     \centering
%                     \subcaption*{\small Ours}
%                 \end{minipage}
%                 \begin{minipage}{.19\textwidth}
%                     \centering
%                     \subcaption*{\small 3DGS-MCMC }
%                 \end{minipage}
%                 \begin{minipage}{.19\textwidth}
%                     \centering
%                     \subcaption*{\small DBS}
%                 \end{minipage}
%                 \begin{minipage}{.19\textwidth}
%                     \centering
%                     \subcaption*{\small SSS}
%                 \end{minipage}
%             \end{minipage}
%         \end{minipage}       
%     \end{minipage}

%     \begin{minipage}{\textwidth}
%         \begin{minipage}{0.03in}	
%             \centering
%             \rotatebox{90}{\small \textsc{room}}
%         \end{minipage}
%         \begin{minipage}{\textwidth}
%             \centering
%             \begin{minipage}{.19\textwidth}
%                 \includegraphics[width=\textwidth]{imgs/comparison/room/room_gt.png}
%                 \put(-13,3){\scalebox{.8}{\color{black} 0.9}}
%             \end{minipage}
%             \begin{minipage}{.19\textwidth}
%                 \includegraphics[width=\textwidth]{imgs/comparison/room/room_our.png}
%                 \put(-13,3){\scalebox{.8}{\color{black} 0.9}}
%             \end{minipage}
%             \begin{minipage}{.19\textwidth}
%                 \includegraphics[width=\textwidth]{imgs/comparison/room/room_mcmc.png}
%                 \put(-13,3){\scalebox{.8}{\color{black} 0.9}}
%             \end{minipage}
%             \begin{minipage}{.19\textwidth}
%                 \includegraphics[width=\textwidth]{imgs/comparison/room/room_beta.png}
%                 \put(-16,3){\scalebox{.8}{\color{black} 48.7}}
%             \end{minipage}
%             \begin{minipage}{.19\textwidth}
%                 \includegraphics[width=\textwidth]{imgs/comparison/room/room_sss.png}
%                 \put(-16,3){\scalebox{.8}{\color{black} 0.93}}
%             \end{minipage}
%         \end{minipage}
%     \end{minipage}

%     % \begin{minipage}{\textwidth}
%     %     \begin{minipage}{0.03in}	
%     %         \centering
%     %         \rotatebox{90}{\small \textsc{owl}}
%     %     \end{minipage}
%     %     \begin{minipage}{\textwidth}
%     %         \centering
%     %         \begin{minipage}{.19\textwidth}
%     %             \includegraphics[width=\textwidth]{imgs/geo_main/owl/our_depth.png}
%     %             \put(-13,3){\scalebox{.8}{\color{black} 6.2}}
%     %         \end{minipage}
%     %         \begin{minipage}{.19\textwidth}
%     %             \includegraphics[width=\textwidth]{imgs/geo_main/owl/xxm_depth.png}
%     %             \put(-13,3){\scalebox{.8}{\color{black} 6.2}}
%     %         \end{minipage}
%     %         \begin{minipage}{.19\textwidth}
%     %             \includegraphics[width=\textwidth]{imgs/geo_main/owl/mps_depth.png}
%     %             \put(-13,3){\scalebox{.8}{\color{black} 6.2}}
%     %         \end{minipage}
%     %         \begin{minipage}{.19\textwidth}
%     %             \includegraphics[width=\textwidth]{imgs/geo_main/owl/gt_2.png}
%     %             \put(-13,3){\scalebox{.8}{\color{black} 6.2}}
%     %         \end{minipage}
%     %         \begin{minipage}{.19\textwidth}
%     %             \includegraphics[width=\textwidth]{imgs/geo_main/owl/our_relight_2.png}
%     %             \put(-16,3){\scalebox{.8}{\color{black} 78.0}}
%     %         \end{minipage}
%     %         \begin{minipage}{.19\textwidth}
%     %             \includegraphics[width=\textwidth]{imgs/geo_main/owl/gt_1.png}
%     %             \put(-16,3){\scalebox{.8}{\color{black} 15.4}}
%     %         \end{minipage}
%     %         \begin{minipage}{.19\textwidth}
%     %             \includegraphics[width=\textwidth]{imgs/geo_main/owl/our_relight_1.png}
%     %             \put(-16,3){\scalebox{.8}{\color{black} 20.0}}
%     %         \end{minipage}
%     %     \end{minipage}
%     % \end{minipage}

%     % \begin{minipage}{\textwidth}
%     %     \begin{minipage}{0.03in}
%     %         \hspace{0.03in}
%     %     \end{minipage}	
%     %     \captionsetup[subfigure]{justification=centering}
%     %     \begin{minipage}{\textwidth}
%     %         \centering
%     %         \begin{minipage}{\textwidth}
%     %             \centering
%     %             \begin{minipage}{.19\textwidth}
%     %                 \centering
%     %                 \subcaption*{\small BP(0.5)=0.72 / BP(1.0)=\textbf{0.93}}
%     %             \end{minipage}
%     %             \begin{minipage}{.19\textwidth}
%     %                 \centering
%     %                 \subcaption*{\small BP(0.5)=\textbf{0.79} / BP(1.0)=0.92}
%     %             \end{minipage}
%     %             \begin{minipage}{.19\textwidth}
%     %                 \centering
%     %                 \subcaption*{\small BP(0.5)=0.48 / BP(1.0)=0.79}
%     %             \end{minipage}
%     %             \begin{minipage}{.19\textwidth}
%     %                 \centering
%     %                 \subcaption*{\small  }
%     %             \end{minipage}
%     %             \begin{minipage}{.19\textwidth}
%     %                 \centering
%     %                 \subcaption*{\small SSIM = 0.93 }
%     %             \end{minipage}
%     %             \begin{minipage}{.19\textwidth}
%     %                 \centering
%     %                 \subcaption*{\small }
%     %             \end{minipage}
%     %             \begin{minipage}{.19\textwidth}
%     %                 \centering
%     %                 \subcaption*{\small SSIM = 0.94 }
%     %             \end{minipage}
%     %         \end{minipage}
%     %     \end{minipage}       
%     % \end{minipage}


%     % \begin{minipage}{\textwidth}
%     %     \begin{minipage}{0.03in}	
%     %         \centering
%     %         \rotatebox{90}{\small \textsc{Container}}
%     %     \end{minipage}
%     %     \begin{minipage}{\textwidth}
%     %         \centering
%     %         \begin{minipage}{.19\textwidth}
%     %             \includegraphics[width=\textwidth]{imgs/geo_main/container/our_depth.png}
%     %             \put(-13,3){\scalebox{.8}{\color{black} 6.2}}
%     %         \end{minipage}
%     %         \begin{minipage}{.19\textwidth}
%     %             \includegraphics[width=\textwidth]{imgs/geo_main/container/xxm_depth.png}
%     %             \put(-13,3){\scalebox{.8}{\color{black} 6.2}}
%     %         \end{minipage}
%     %         \begin{minipage}{.19\textwidth}
%     %             \includegraphics[width=\textwidth]{imgs/geo_main/container/mps_depth.png}
%     %             \put(-13,3){\scalebox{.8}{\color{black} 6.2}}
%     %         \end{minipage}
%     %         \begin{minipage}{.19\textwidth}
%     %             \includegraphics[width=\textwidth]{imgs/geo_main/container/gt_0.png}
%     %             \put(-13,3){\scalebox{.8}{\color{black} 6.2}}
%     %         \end{minipage}
%     %         \begin{minipage}{.19\textwidth}
%     %             \includegraphics[width=\textwidth]{imgs/geo_main/container/our_relight_0.png}
%     %             \put(-16,3){\scalebox{.8}{\color{black} 78.0}}
%     %         \end{minipage}
%     %         \begin{minipage}{.19\textwidth}
%     %             \includegraphics[width=\textwidth]{imgs/geo_main/container/gt_1.png}
%     %             \put(-16,3){\scalebox{.8}{\color{black} 15.4}}
%     %         \end{minipage}
%     %         \begin{minipage}{.19\textwidth}
%     %             \includegraphics[width=\textwidth]{imgs/geo_main/container/our_relight_1.png}
%     %             \put(-16,3){\scalebox{.8}{\color{black} 20.0}}
%     %         \end{minipage}
%     %     \end{minipage}
%     % \end{minipage}

%     % \begin{minipage}{\textwidth}
%     %     \begin{minipage}{0.03in}
%     %         \hspace{0.03in}
%     %     \end{minipage}	
%     %     \captionsetup[subfigure]{justification=centering}
%     %     \begin{minipage}{\textwidth}
%     %         \centering
%     %         \begin{minipage}{\textwidth}
%     %             \centering
%     %             \begin{minipage}{.19\textwidth}
%     %                 \centering
%     %                 \subcaption*{\small BP(0.5)=\textbf{0.71} / BP(1.0)=\textbf{0.88}}
%     %             \end{minipage}
%     %             \begin{minipage}{.19\textwidth}
%     %                 \centering
%     %                 \subcaption*{\small BP(0.5)=0.54 / BP(1.0)=0.74}
%     %             \end{minipage}
%     %             \begin{minipage}{.19\textwidth}
%     %                 \centering
%     %                 \subcaption*{\small BP(0.5)=0.40 / BP(1.0)=0.65}
%     %             \end{minipage}
%     %             \begin{minipage}{.19\textwidth}
%     %                 \centering
%     %                 \subcaption*{\small  }
%     %             \end{minipage}
%     %             \begin{minipage}{.19\textwidth}
%     %                 \centering
%     %                 \subcaption*{\small SSIM = 0.92 }
%     %             \end{minipage}
%     %             \begin{minipage}{.19\textwidth}
%     %                 \centering
%     %                 \subcaption*{\small }
%     %             \end{minipage}
%     %             \begin{minipage}{.19\textwidth}
%     %                 \centering
%     %                 \subcaption*{\small SSIM = 0.93 }
%     %             \end{minipage}
%     %         \end{minipage}
%     %     \end{minipage}       
%     % \end{minipage}

%     \begin{minipage}{\textwidth}
%         \begin{minipage}{0.03in}	
%             \centering
%             \rotatebox{90}{\small \textsc{Bonsai}}
%         \end{minipage}
%         \begin{minipage}{\textwidth}
%             \centering
%             \begin{minipage}{.19\textwidth}
%                 \includegraphics[width=\textwidth]{imgs/comparison/bonsai/bonsai_gt_26.png}
%                 \put(-13,3){\scalebox{.8}{\color{black} 6.2}}
%             \end{minipage}
%             \begin{minipage}{.19\textwidth}
%                 \includegraphics[width=\textwidth]{imgs/comparison/bonsai/bonsai_our_26.png}
%                 \put(-13,3){\scalebox{.8}{\color{black} 6.2}}
%             \end{minipage}
%             \begin{minipage}{.19\textwidth}
%                 \includegraphics[width=\textwidth]{imgs/comparison/bonsai/bonsai_mcmc_26.png}
%                 \put(-16,3){\scalebox{.8}{\color{black} 78.0}}
%             \end{minipage}
%             \begin{minipage}{.19\textwidth}
%                 \includegraphics[width=\textwidth]{imgs/comparison/bonsai/bonsai_beta_26.png}
%                 \put(-16,3){\scalebox{.8}{\color{black} 15.4}}
%             \end{minipage}
%             \begin{minipage}{.19\textwidth}
%                 \includegraphics[width=\textwidth]{imgs/comparison/bonsai/bonsai_sss_26.png}
%                 \put(-16,3){\scalebox{.8}{\color{black} 20.0}}
%             \end{minipage}
%         \end{minipage}
%     \end{minipage}

%     \begin{minipage}{\textwidth}
%         \begin{minipage}{0.03in}	
%             \centering
%             \rotatebox{90}{\small \textsc{Train}}
%         \end{minipage}
%         \begin{minipage}{\textwidth}
%             \centering
%             \begin{minipage}{.19\textwidth}
%                 \includegraphics[width=\textwidth]{imgs/comparison/train/train_gt_34.png}
%                 \put(-13,3){\scalebox{.8}{\color{black} 6.2}}
%             \end{minipage}
%             \begin{minipage}{.19\textwidth}
%                 \includegraphics[width=\textwidth]{imgs/comparison/train/train_our_34.png}
%                 \put(-13,3){\scalebox{.8}{\color{black} 6.2}}
%             \end{minipage}
%             \begin{minipage}{.19\textwidth}
%                 \includegraphics[width=\textwidth]{imgs/comparison/train/train_mcmc_34.png}
%                 \put(-13,3){\scalebox{.8}{\color{black} 6.2}}
%             \end{minipage}
%             \begin{minipage}{.19\textwidth}
%                 \includegraphics[width=\textwidth]{imgs/comparison/train/train_beta_34.png}
%                 \put(-16,3){\scalebox{.8}{\color{black} 15.4}}
%             \end{minipage}
%             \begin{minipage}{.19\textwidth}
%                 \includegraphics[width=\textwidth]{imgs/comparison/train/train_sss_34.png}
%                 \put(-16,3){\scalebox{.8}{\color{black} 20.0}}
%             \end{minipage}
%         \end{minipage}
%     \end{minipage}
%     \begin{minipage}{\textwidth}
%         \begin{minipage}{0.03in}	
%             \centering
%             \rotatebox{90}{\small \textsc{Playroom}}
%         \end{minipage}
%         \begin{minipage}{\textwidth}
%             \centering
%             \begin{minipage}{.19\textwidth}
%                 \includegraphics[width=\textwidth]{imgs/comparison/playroom/playroom_gt_06.png}
%                 \put(-13,3){\scalebox{.8}{\color{black} 6.2}}
%             \end{minipage}
%             \begin{minipage}{.19\textwidth}
%                 \includegraphics[width=\textwidth]{imgs/comparison/playroom/playroom_our_06.png}
%                 \put(-13,3){\scalebox{.8}{\color{black} 6.2}}
%             \end{minipage}
%             \begin{minipage}{.19\textwidth}
%                 \includegraphics[width=\textwidth]{imgs/comparison/playroom/playroom_mcmc_06.png}
%                 \put(-16,3){\scalebox{.8}{\color{black} 78.0}}
%             \end{minipage}
%             \begin{minipage}{.19\textwidth}
%                 \includegraphics[width=\textwidth]{imgs/comparison/playroom/playroom_beta_06.png}
%                 \put(-16,3){\scalebox{.8}{\color{black} 15.4}}
%             \end{minipage}
%             \begin{minipage}{.19\textwidth}
%                 \includegraphics[width=\textwidth]{imgs/comparison/playroom/playroom_sss_06.png}
%                 \put(-16,3){\scalebox{.8}{\color{black} 20.0}}
%             \end{minipage}
%         \end{minipage}
%     \end{minipage}

%   \begin{minipage}{\textwidth}
%         \begin{minipage}{0.03in}	
%             \centering
%             \rotatebox{90}{\small \textsc{scene5}}
%         \end{minipage}
%         \begin{minipage}{\textwidth}
%             \centering
%             \begin{minipage}{.19\textwidth}
%                 \includegraphics[width=\textwidth]{example-image-duck}
%                 \put(-13,3){\scalebox{.8}{\color{black} 6.2}}
%             \end{minipage}
%             \begin{minipage}{.19\textwidth}
%                 \includegraphics[width=\textwidth]{example-image-duck}
%                 \put(-13,3){\scalebox{.8}{\color{black} 6.2}}
%             \end{minipage}
%             \begin{minipage}{.19\textwidth}
%                 \includegraphics[width=\textwidth]{example-image-duck}
%                 \put(-16,3){\scalebox{.8}{\color{black} 78.0}}
%             \end{minipage}
%             \begin{minipage}{.19\textwidth}
%                 \includegraphics[width=\textwidth]{example-image-duck}
%                 \put(-16,3){\scalebox{.8}{\color{black} 15.4}}
%             \end{minipage}
%             \begin{minipage}{.19\textwidth}
%                 \includegraphics[width=\textwidth]{example-image-duck}
%                 \put(-16,3){\scalebox{.8}{\color{black} 20.0}}
%             \end{minipage}
%         \end{minipage}
%     \end{minipage}
%     \caption{Qualitative comparisons with state-of-the-art techniques.}
%     \Description{A figure showing qualitative comparisons with state-of-the-art techniques.}
%     \label{fig:main}
% \end{figure*}

==> fig/main_comparison_subfigure.tex <==
% \begin{figure*}[htbp]
%     \centering
%     \captionsetup[subfigure]{justification=centering}

%     % ==========================
%     % 1. 标题行 (Header Row)
%     % ==========================
%     \begin{minipage}{\textwidth}
%         \begin{minipage}{0.10in}
%             \hspace{0.03in} % 对应左侧标签占位
%         \end{minipage}  
%         % 除去左侧标签后的区域
%         \begin{minipage}{\dimexpr\textwidth-0.03in-1em\relax}
%             \centering
%             % GT 列：宽度设为其它列的3倍 (约 0.32)
%             \begin{minipage}{.32\linewidth} \centering \subcaption*{\small GT} \end{minipage}%
%             \hfill
%             % 其余列：宽度 (约 0.16)
%             \begin{minipage}{.16\linewidth} \centering \subcaption*{\small Ours} \end{minipage}%
%             \hfill
%             \begin{minipage}{.16\linewidth} \centering \subcaption*{\small 3DGS-MCMC} \end{minipage}%
%             \hfill
%             \begin{minipage}{.16\linewidth} \centering \subcaption*{\small DBS} \end{minipage}%
%             \hfill
%             \begin{minipage}{.16\linewidth} \centering \subcaption*{\small SSS} \end{minipage}
%         \end{minipage}       
%     \end{minipage}
    
%     \vspace{2pt} 

%     % ==========================
%     % 2. 第一行数据 (Room)
%     % ==========================
%     \begin{minipage}{\textwidth}
%         % --- 左侧竖排标签 ---
%         \begin{minipage}[t]{0.10in}    
%             \vspace{0pt}
%             \centering
%             % 垂直居中调整：由于右侧列变高了(含子图)，标签可能需要往下挪一点
%             \vspace{0.6in} 
%             \rotatebox{90}{\small \textsc{Room}}
%         \end{minipage}
%         % --- 右侧图片内容 ---
%         \begin{minipage}[t]{\dimexpr\textwidth-0.03in-1em\relax}
%             \vspace{0pt}
%             \centering
            
%             % [第1列 GT]
%             % 宽度 0.32，长宽比3:1。因此高度 = 0.32宽度 / 3 = 0.16宽度
%             % 这与后面几列的主图(1:1, 宽度0.16)高度完全一致
%             \begin{minipage}[t]{.32\linewidth}
%                 \vspace{0pt}
%                 \centering
%                 % 确保这张图原图比例是 3:1
%                 \includegraphics[width=\linewidth, height=0.66\linewidth]{imgs/comparison/room/room_gt.png}
%                 % GT通常不需要指标，如果需要可自行加 \put
%             \end{minipage}%
%             \hfill
%             % [第2列 Ours]
%             \begin{minipage}[t]{.16\linewidth}
%                 \vspace{0pt}
%                 \centering
%                 % 主图 (1:1)
%                 \includegraphics[width=\linewidth, height=\linewidth]{imgs/comparison/room/crop_room_our_16.png}
%                 \put(-13,3){\scalebox{.6}{\color{black} 0.9}} % 字号稍微改小以适应窄列
%                 \vspace{1.5pt} 
%                 % 子图 (3张)
%                 % 0.32 * 0.16\textwidth 实际上很小，保证清晰度
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{imgs/comparison/room/room_0_2732.pdf}\hfill
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{imgs/comparison/room/room_1_9845.pdf}\hfill
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{imgs/comparison/room/room.pdf}
%             \end{minipage}%
%             \hfill
%             % [第3列 MCMC]
%             \begin{minipage}[t]{.16\linewidth}
%                 \vspace{0pt}
%                 \centering
%                 \includegraphics[width=\linewidth, height=\linewidth]{imgs/comparison/room/crop_room_mcmc_16.png}
%                 \put(-13,3){\scalebox{.6}{\color{black} 0.9}}
%                 \vspace{1.5pt}
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{imgs/comparison/room/gs_curve_2732.pdf}\hfill
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{example-image-duck}\hfill
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{example-image-duck}
%             \end{minipage}%
%             \hfill
%             % [第4列 DBS]
%             \begin{minipage}[t]{.16\linewidth}
%                 \vspace{0pt}
%                 \centering
%                 \includegraphics[width=\linewidth, height=\linewidth]{imgs/comparison/room/crop_room_beta_16.png}
%                 \put(-13,3){\scalebox{.6}{\color{black} 48}}
%                 \vspace{1.5pt}
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{imgs/comparison/room/beta_curve_2732.pdf}\hfill
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{example-image-duck}\hfill
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{example-image-duck}
%             \end{minipage}%
%             \hfill
%             % [第5列 SSS]
%             \begin{minipage}[t]{.16\linewidth}
%                 \vspace{0pt}
%                 \centering
%                 \includegraphics[width=\linewidth, height=\linewidth]{imgs/comparison/room/crop_room_sss_16.png}
%                 \put(-13,3){\scalebox{.6}{\color{black} 0.9}}
%                 \vspace{1.5pt}
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{imgs/comparison/room/sss_curve_2732.pdf}\hfill
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{example-image-duck}\hfill
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{example-image-duck}
%             \end{minipage}
%         \end{minipage}
%     \end{minipage}

%     \vspace{4pt} % 行间距

%     % ==========================
%     % 2. 第一行数据 (Room)
%     % ==========================
%     \begin{minipage}{\textwidth}
%         % --- 左侧竖排标签 ---
%         \begin{minipage}[t]{0.10in}    
%             \vspace{0pt}
%             \centering
%             % 垂直居中调整：由于右侧列变高了(含子图)，标签可能需要往下挪一点
%             \vspace{0.6in} 
%             \rotatebox{90}{\small \textsc{Bonsai}}
%         \end{minipage}
%         % --- 右侧图片内容 ---
%         \begin{minipage}[t]{\dimexpr\textwidth-0.03in-1em\relax}
%             \vspace{0pt}
%             \centering
            
%             % [第1列 GT]
%             % 宽度 0.32，长宽比3:1。因此高度 = 0.32宽度 / 3 = 0.16宽度
%             % 这与后面几列的主图(1:1, 宽度0.16)高度完全一致
%             \begin{minipage}[t]{.32\linewidth}
%                 \vspace{0pt}
%                 \centering
%                 % 确保这张图原图比例是 3:1
%                 \includegraphics[width=\linewidth, height=0.66\linewidth]{imgs/comparison/bonsai/bonsai_gt_26.png}
%                 % GT通常不需要指标，如果需要可自行加 \put
%             \end{minipage}%
%             \hfill
%             % [第2列 Ours]
%             \begin{minipage}[t]{.16\linewidth}
%                 \vspace{0pt}
%                 \centering
%                 % 主图 (1:1)
%                 \includegraphics[width=\linewidth, height=\linewidth]{imgs/comparison/bonsai/crop_bonsai_our_26.png}
%                 \put(-13,3){\scalebox{.6}{\color{black} 0.9}} % 字号稍微改小以适应窄列
%                 \vspace{1.5pt} 
%                 % 子图 (3张)
%                 % 0.32 * 0.16\textwidth 实际上很小，保证清晰度
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{imgs/comparison/room/room_0_2732.pdf}\hfill
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{imgs/comparison/room/room_1_9845.pdf}\hfill
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{imgs/comparison/room/room.pdf}
%             \end{minipage}%
%             \hfill
%             % [第3列 MCMC]
%             \begin{minipage}[t]{.16\linewidth}
%                 \vspace{0pt}
%                 \centering
%                 \includegraphics[width=\linewidth, height=\linewidth]{imgs/comparison/bonsai/crop_bonsai_mcmc_26.png}
%                 \put(-13,3){\scalebox{.6}{\color{black} 0.9}}
%                 \vspace{1.5pt}
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{imgs/comparison/room/gs_curve_2732.pdf}\hfill
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{example-image-duck}\hfill
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{example-image-duck}
%             \end{minipage}%
%             \hfill
%             % [第4列 DBS]
%             \begin{minipage}[t]{.16\linewidth}
%                 \vspace{0pt}
%                 \centering
%                 \includegraphics[width=\linewidth, height=\linewidth]{imgs/comparison/bonsai/crop_bonsai_beta_26.png}
%                 \put(-13,3){\scalebox{.6}{\color{black} 48}}
%                 \vspace{1.5pt}
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{imgs/comparison/room/beta_curve_2732.pdf}\hfill
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{example-image-duck}\hfill
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{example-image-duck}
%             \end{minipage}%
%             \hfill
%             % [第5列 SSS]
%             \begin{minipage}[t]{.16\linewidth}
%                 \vspace{0pt}
%                 \centering
%                 \includegraphics[width=\linewidth, height=\linewidth]{imgs/comparison/bonsai/crop_bonsai_sss_26.png}
%                 \put(-13,3){\scalebox{.6}{\color{black} 0.9}}
%                 \vspace{1.5pt}
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{imgs/comparison/room/sss_curve_2732.pdf}\hfill
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{example-image-duck}\hfill
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{example-image-duck}
%             \end{minipage}
%         \end{minipage}
%     \end{minipage}

%     \vspace{4pt} % 行间距

%         % ==========================
%     % 2. 第一行数据 (Room)
%     % ==========================
%     \begin{minipage}{\textwidth}
%         % --- 左侧竖排标签 ---
%         \begin{minipage}[t]{0.10in}    
%             \vspace{0pt}
%             \centering
%             % 垂直居中调整：由于右侧列变高了(含子图)，标签可能需要往下挪一点
%             \vspace{0.6in} 
%             \rotatebox{90}{\small \textsc{Train}}
%         \end{minipage}
%         % --- 右侧图片内容 ---
%         \begin{minipage}[t]{\dimexpr\textwidth-0.03in-1em\relax}
%             \vspace{0pt}
%             \centering
            
%             % [第1列 GT]
%             % 宽度 0.32，长宽比3:1。因此高度 = 0.32宽度 / 3 = 0.16宽度
%             % 这与后面几列的主图(1:1, 宽度0.16)高度完全一致
%             \begin{minipage}[t]{.32\linewidth}
%                 \vspace{0pt}
%                 \centering
%                 % 确保这张图原图比例是 3:1
%                 \includegraphics[width=\linewidth, height=0.66\linewidth]{imgs/comparison/train/train_gt_34.png}
%                 % GT通常不需要指标，如果需要可自行加 \put
%             \end{minipage}%
%             \hfill
%             % [第2列 Ours]
%             \begin{minipage}[t]{.16\linewidth}
%                 \vspace{0pt}
%                 \centering
%                 % 主图 (1:1)
%                 \includegraphics[width=\linewidth, height=\linewidth]{imgs/comparison/train/crop_train_our_34.png}
%                 \put(-13,3){\scalebox{.6}{\color{black} 0.9}} % 字号稍微改小以适应窄列
%                 \vspace{1.5pt} 
%                 % 子图 (3张)
%                 % 0.32 * 0.16\textwidth 实际上很小，保证清晰度
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{imgs/comparison/room/room_0_2732.pdf}\hfill
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{imgs/comparison/room/room_1_9845.pdf}\hfill
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{imgs/comparison/room/room.pdf}
%             \end{minipage}%
%             \hfill
%             % [第3列 MCMC]
%             \begin{minipage}[t]{.16\linewidth}
%                 \vspace{0pt}
%                 \centering
%                 \includegraphics[width=\linewidth, height=\linewidth]{imgs/comparison/train/crop_train_mcmc_34.png}
%                 \put(-13,3){\scalebox{.6}{\color{black} 0.9}}
%                 \vspace{1.5pt}
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{imgs/comparison/room/gs_curve_2732.pdf}\hfill
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{example-image-duck}\hfill
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{example-image-duck}
%             \end{minipage}%
%             \hfill
%             % [第4列 DBS]
%             \begin{minipage}[t]{.16\linewidth}
%                 \vspace{0pt}
%                 \centering
%                 \includegraphics[width=\linewidth, height=\linewidth]{imgs/comparison/train/crop_train_beta_34.png}
%                 \put(-13,3){\scalebox{.6}{\color{black} 48}}
%                 \vspace{1.5pt}
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{imgs/comparison/room/beta_curve_2732.pdf}\hfill
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{example-image-duck}\hfill
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{example-image-duck}
%             \end{minipage}%
%             \hfill
%             % [第5列 SSS]
%             \begin{minipage}[t]{.16\linewidth}
%                 \vspace{0pt}
%                 \centering
%                 \includegraphics[width=\linewidth, height=\linewidth]{imgs/comparison/train/crop_train_sss_34.png}
%                 \put(-13,3){\scalebox{.6}{\color{black} 0.9}}
%                 \vspace{1.5pt}
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{imgs/comparison/room/sss_curve_2732.pdf}\hfill
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{example-image-duck}\hfill
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{example-image-duck}
%             \end{minipage}
%         \end{minipage}
%     \end{minipage}

%     \vspace{4pt} % 行间距

%         % ==========================
%     % 2. 第一行数据 (Room)
%     % ==========================
%     \begin{minipage}{\textwidth}
%         % --- 左侧竖排标签 ---
%         \begin{minipage}[t]{0.10in}    
%             \vspace{0pt}
%             \centering
%             % 垂直居中调整：由于右侧列变高了(含子图)，标签可能需要往下挪一点
%             \vspace{0.6in} 
%             \rotatebox{90}{\small \textsc{Playroom}}
%         \end{minipage}
%         % --- 右侧图片内容 ---
%         \begin{minipage}[t]{\dimexpr\textwidth-0.03in-1em\relax}
%             \vspace{0pt}
%             \centering
            
%             % [第1列 GT]
%             % 宽度 0.32，长宽比3:1。因此高度 = 0.32宽度 / 3 = 0.16宽度
%             % 这与后面几列的主图(1:1, 宽度0.16)高度完全一致
%             \begin{minipage}[t]{.32\linewidth}
%                 \vspace{0pt}
%                 \centering
%                 % 确保这张图原图比例是 3:1
%                 \includegraphics[width=\linewidth, height=0.66\linewidth]{imgs/comparison/playroom/playroom_gt_06.png}
%                 % GT通常不需要指标，如果需要可自行加 \put
%             \end{minipage}%
%             \hfill
%             % [第2列 Ours]
%             \begin{minipage}[t]{.16\linewidth}
%                 \vspace{0pt}
%                 \centering
%                 % 主图 (1:1)
%                 \includegraphics[width=\linewidth, height=\linewidth]{imgs/comparison/playroom/crop_playroom_our_06.png}
%                 \put(-13,3){\scalebox{.6}{\color{black} 0.9}} % 字号稍微改小以适应窄列
%                 \vspace{1.5pt} 
%                 % 子图 (3张)
%                 % 0.32 * 0.16\textwidth 实际上很小，保证清晰度
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{imgs/comparison/room/room_0_2732.pdf}\hfill
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{imgs/comparison/room/room_1_9845.pdf}\hfill
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{imgs/comparison/room/room.pdf}
%             \end{minipage}%
%             \hfill
%             % [第3列 MCMC]
%             \begin{minipage}[t]{.16\linewidth}
%                 \vspace{0pt}
%                 \centering
%                 \includegraphics[width=\linewidth, height=\linewidth]{imgs/comparison/playroom/crop_playroom_mcmc_06.png}
%                 \put(-13,3){\scalebox{.6}{\color{black} 0.9}}
%                 \vspace{1.5pt}
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{imgs/comparison/room/gs_curve_2732.pdf}\hfill
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{example-image-duck}\hfill
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{example-image-duck}
%             \end{minipage}%
%             \hfill
%             % [第4列 DBS]
%             \begin{minipage}[t]{.16\linewidth}
%                 \vspace{0pt}
%                 \centering
%                 \includegraphics[width=\linewidth, height=\linewidth]{imgs/comparison/playroom/crop_playroom_beta_06.png}
%                 \put(-13,3){\scalebox{.6}{\color{black} 48}}
%                 \vspace{1.5pt}
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{imgs/comparison/room/beta_curve_2732.pdf}\hfill
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{example-image-duck}\hfill
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{example-image-duck}
%             \end{minipage}%
%             \hfill
%             % [第5列 SSS]
%             \begin{minipage}[t]{.16\linewidth}
%                 \vspace{0pt}
%                 \centering
%                 \includegraphics[width=\linewidth, height=\linewidth]{imgs/comparison/playroom/crop_playroom_sss_06.png}
%                 \put(-13,3){\scalebox{.6}{\color{black} 0.9}}
%                 \vspace{1.5pt}
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{imgs/comparison/room/sss_curve_2732.pdf}\hfill
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{example-image-duck}\hfill
%                 \includegraphics[width=0.32\linewidth, height=0.32\linewidth]{example-image-duck}
%             \end{minipage}
%         \end{minipage}
%     \end{minipage}

%     \vspace{4pt} % 行间距


%     % ... 复制上方 Scene2 的块并修改图片路径即可 ...

%     \caption{Qualitative comparisons with state-of-the-art techniques. For each model, we take three primitives and visualize their kernel shapes under different views, which are drawn from light to dark and superimposed to indicate the trajectory. }
%     \label{fig:main}
% \end{figure*}

==> fig/training_progress.tex <==
% \begin{figure}[htbp]
%     \centering
%     \captionsetup[subfigure]{justification=centering}

%     % --- 第一列 (Initial) ---
%     \begin{minipage}[t]{0.32\linewidth}
%         \centering
%         % 1. 标题
%         \subcaption*{\small Initial}
%         \vspace{2pt}
        
%         % 2. 大图
%         \includegraphics[width=\linewidth]{imgs/process/1000.png}
        
%         % 3. 该图对应的子图 (假设每张大图下有3张小图)
%         % 小图宽度设为 0.32\linewidth 是相对于当前这个minipage的宽度的
%         \includegraphics[width=0.32\linewidth]{imgs/visualization/our.png}\hfill
%         \includegraphics[width=0.32\linewidth]{imgs/visualization/our.png}\hfill
%         \includegraphics[width=0.32\linewidth]{imgs/visualization/our.png}
%     \end{minipage}
%     \hfill % 列之间的弹性间距
%     % --- 第二列 (5000 it) ---
%     \begin{minipage}[t]{0.32\linewidth}
%         \centering
%         % 1. 标题
%         \subcaption*{\small 5000 it}
%         \vspace{2pt}
        
%         % 2. 大图
%         \includegraphics[width=\linewidth]{imgs/process/1000.png}
        
%         % 3. 该图对应的子图
%         \includegraphics[width=0.32\linewidth]{imgs/visualization/our.png}\hfill
%         \includegraphics[width=0.32\linewidth]{imgs/visualization/our.png}\hfill
%         \includegraphics[width=0.32\linewidth]{imgs/visualization/our.png}
%     \end{minipage}
%     \hfill
%     % --- 第三列 (Final) ---
%     \begin{minipage}[t]{0.32\linewidth}
%         \centering
%         % 1. 标题
%         \subcaption*{\small Final}
%         \vspace{2pt}
        
%         % 2. 大图
%         \includegraphics[width=\linewidth]{imgs/process/1000.png}
        
%         % 3. 该图对应的子图
%         \includegraphics[width=0.32\linewidth]{imgs/visualization/our.png}\hfill
%         \includegraphics[width=0.32\linewidth]{imgs/visualization/our.png}\hfill
%         \includegraphics[width=0.32\linewidth]{imgs/visualization/our.png}
%     \end{minipage}

%     \caption{\textbf{Training Dynamics.} We show the progression of the rendered view (top) and the corresponding evolution of three neural primitives (bottom). Starting from a Gaussian-like initialization, the network iteratively refines the kernel shapes to distinctive, view-aware forms.
%     }    
%     \label{fig:training_progress}
% \end{figure}

==> fig/visualization.tex <==
% \begin{figure*}[htbp]
%     \centering
%     \captionsetup[subfigure]{justification=centering}
%     \begin{minipage}{\linewidth}
%         \centering
%         \begin{minipage}{\textwidth}
%             \centering
%             \begin{minipage}{.155\textwidth}
%                 \centering 
%                 \subcaption*{\small Our-View0}
%             \end{minipage}
%             \begin{minipage}{.155\textwidth}
%                 \centering 
%                 \subcaption*{\small Our-View1}
%             \end{minipage}
%             \begin{minipage}{.155\textwidth}
%                 \centering 
%                 \subcaption*{\small Our-View2}
%             \end{minipage}
%             \begin{minipage}{.155\textwidth}
%                 \centering
%                 \subcaption*{\small Beta}
%             \end{minipage}
%             \begin{minipage}{.155\textwidth}
%                 \centering
%                 \subcaption*{\small Student-t}
%             \end{minipage}
%             \begin{minipage}{.155\textwidth}
%                 \centering
%                 \subcaption*{\small Gaussian}
%             \end{minipage}
%             % \begin{minipage}{.1555\textwidth}
%             %     \centering
%             %     \subcaption*{\small Per-pixel Loss}
%             % \end{minipage}
%         \end{minipage}
%     \end{minipage}  
%     % \begin{minipage}{\linewidth}
%     %     \centering
%     %     \begin{minipage}{.19\linewidth}
%     %         \centering
%     %         \subcaption*{\small LightPattern}
%     %     \end{minipage}
%     %     \begin{minipage}{.19\linewidth}
%     %         \centering
%     %         \subcaption*{\small MaskPattern}
%     %     \end{minipage}
%     %     \begin{minipage}{.19\linewidth}
%     %         \centering
%     %         \subcaption*{\small Photograph}
%     %     \end{minipage}
%     %     \begin{minipage}{.19\linewidth}
%     %         \centering
%     %         \subcaption*{\small DepthUncertainty}
%     %     \end{minipage}
%     % \end{minipage}
%     \begin{minipage}{\linewidth}
%         \centering
%         \begin{minipage}{.155\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{imgs/visualization/our.png}
%         \end{minipage}
%         \begin{minipage}{.155\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{imgs/visualization/our.png}
%         \end{minipage}
%         \begin{minipage}{.155\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{imgs/visualization/our.png}
%         \end{minipage}
%         \begin{minipage}{.155\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{imgs/visualization/beta.png}
%         \end{minipage}
%         \begin{minipage}{.155\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{imgs/visualization/sss.png}
%         \end{minipage}
%          \begin{minipage}{.155\linewidth}
%             \centering
%             \includegraphics[width=\linewidth]{imgs/visualization/gaussian.png}
%         \end{minipage}
%     \end{minipage}



%     \caption{Visualization.}   
%     \label{fig:visualization}
% \end{figure*}


